An incompressible Eulerian method for fluid-structure interaction with mixed soft and rigid solids

We present a general simulation approach for incompressible fluid--structure interactions in a fully Eulerian framework using the reference map technique (RMT). The approach is suitable for modeling one or more rigid or finitely-deformable objects or soft objects with rigid components interacting with the fluid and with each other. It is also extended to control the kinematics of structures in fluids. The model is based on our previous Eulerian fluid--soft solver, and generalized to rigid structures by constraining the deformation-rate tensor in a projection framework. Several numerical examples are presented to illustrate the capability of the method.

==> conv-test.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9123.84,4147.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(825,552){\makebox(0,0)[r]{\strut{}$10^{-3}$}}%
      \put(825,1424){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(825,2296){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \put(825,3168){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(1323,392){\makebox(0,0){\strut{}$\frac{1}{400}$}}%
      \put(2570,392){\makebox(0,0){\strut{}$\frac{1}{200}$}}%
      \put(3818,392){\makebox(0,0){\strut{}$\frac{1}{100}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(169,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Error: $\|\mathbf{v}-\mathbf{v}_{ref}\|_2$}}}%
      \put(2533,72){\makebox(0,0){\strut{}$\Delta x$}}%
      \put(613,4178){\makebox(0,0){\strut{}(a)}}%
      \csname LTb\endcsname%
      \put(3411,3595){\makebox(0,0)[r]{\strut{}standard}}%
      \csname LTb\endcsname%
      \put(3411,3355){\makebox(0,0)[r]{\strut{}constant blur}}%
      \csname LTb\endcsname%
      \put(2534,2004){\makebox(0,0)[l]{\strut{}p=2}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5433,552){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(5433,1424){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \put(5433,2296){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(5433,3168){\makebox(0,0)[r]{\strut{}$10^{1}$}}%
      \put(5931,392){\makebox(0,0){\strut{}$\frac{1}{400}$}}%
      \put(7178,392){\makebox(0,0){\strut{}$\frac{1}{200}$}}%
      \put(8426,392){\makebox(0,0){\strut{}$\frac{1}{100}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4777,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Error: $\|\mathbf{v}-\mathbf{v}_{ref}\|_\infty$}}}%
      \put(7141,72){\makebox(0,0){\strut{}$\Delta x$}}%
      \put(5221,4178){\makebox(0,0){\strut{}(b)}}%
      \csname LTb\endcsname%
      \put(8019,3595){\makebox(0,0)[r]{\strut{}standard}}%
      \csname LTb\endcsname%
      \put(8019,3355){\makebox(0,0)[r]{\strut{}constant blur}}%
      \csname LTb\endcsname%
      \put(7142,2165){\makebox(0,0)[l]{\strut{}p=1.5}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{conv-test_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> densitydiff.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9123.84,6451.20)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1747,1475){\makebox(0,0)[r]{\strut{}$-6$}}%
      \put(1747,3010){\makebox(0,0)[r]{\strut{}$-4$}}%
      \put(1747,4546){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(1747,6081){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(2065,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(3095,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1379,3778){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \put(2580,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(1887,5621){\makebox(0,0)[l]{\strut{}\footnotesize$\rho_r/\rho_f=0.1$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3313,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(3313,3010){\makebox(0,0)[r]{\strut{}}}%
      \put(3313,4546){\makebox(0,0)[r]{\strut{}}}%
      \put(3313,6081){\makebox(0,0)[r]{\strut{}}}%
      \put(3631,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(4661,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4146,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(3453,5621){\makebox(0,0)[l]{\strut{}\footnotesize$\rho_r/\rho_f=2.0$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4880,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(4880,3010){\makebox(0,0)[r]{\strut{}}}%
      \put(4880,4546){\makebox(0,0)[r]{\strut{}}}%
      \put(4880,6081){\makebox(0,0)[r]{\strut{}}}%
      \put(5198,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(6228,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5713,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(5020,5621){\makebox(0,0)[l]{\strut{}\footnotesize$\rho_r/\rho_f=5.0$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6447,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(6447,3010){\makebox(0,0)[r]{\strut{}}}%
      \put(6447,4546){\makebox(0,0)[r]{\strut{}}}%
      \put(6447,6081){\makebox(0,0)[r]{\strut{}}}%
      \put(6765,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(7795,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7280,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(6587,5621){\makebox(0,0)[l]{\strut{}\footnotesize$\rho_r/\rho_f=10.0$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2304,385){\makebox(0,0){\strut{}$-300$}}%
      \put(3456,385){\makebox(0,0){\strut{}$-150$}}%
      \put(4608,385){\makebox(0,0){\strut{}$0$}}%
      \put(5759,385){\makebox(0,0){\strut{}$150$}}%
      \put(6911,385){\makebox(0,0){\strut{}$300$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1383,682){\makebox(0,0)[l]{\strut{}$\omega$ (s$^{-1}$)}}%
    }%
    \gplbacktext
    \put(1843,1474){\includegraphics[width=73.7bp,height=230.4bp]{densitydiff_w_01}}%
    \put(3409,1474){\includegraphics[width=73.7bp,height=230.4bp]{densitydiff_w_1}}%
    \put(4976,1474){\includegraphics[width=73.7bp,height=230.4bp]{densitydiff_w_5}}%
    \put(6543,1474){\includegraphics[width=73.7bp,height=230.4bp]{densitydiff_w_10}}%
    \put(2304,552){\includegraphics[width=230.35bp,height=9.25bp]{densitydiff_wbar}}%
    \put(0,0){\includegraphics{densitydiff_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> dkt-traj.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9123.84,5529.60)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(825,615){\makebox(0,0)[r]{\strut{}$-40$}}%
      \put(825,1248){\makebox(0,0)[r]{\strut{}$-30$}}%
      \put(825,1880){\makebox(0,0)[r]{\strut{}$-20$}}%
      \put(825,2513){\makebox(0,0)[r]{\strut{}$-10$}}%
      \put(825,3145){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(825,3778){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(921,392){\makebox(0,0){\strut{}$0$}}%
      \put(1996,392){\makebox(0,0){\strut{}$10$}}%
      \put(3071,392){\makebox(0,0){\strut{}$20$}}%
      \put(4146,392){\makebox(0,0){\strut{}$30$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(265,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Vertical position $y_c/r$}}}%
      \put(2533,72){\makebox(0,0){\strut{}Time $t/\sqrt{r/g}$}}%
      \put(325,4178){\makebox(0,0){\strut{}(a)}}%
      \csname LTb\endcsname%
      \put(3411,3595){\makebox(0,0)[r]{\strut{}Uhlmann leading}}%
      \csname LTb\endcsname%
      \put(3411,3355){\makebox(0,0)[r]{\strut{}Uhlmann trailing}}%
      \csname LTb\endcsname%
      \put(3411,3115){\makebox(0,0)[r]{\strut{}Glowinski leading}}%
      \csname LTb\endcsname%
      \put(3411,2875){\makebox(0,0)[r]{\strut{}Glowinski trailing}}%
      \csname LTb\endcsname%
      \put(3411,2635){\makebox(0,0)[r]{\strut{}Leading}}%
      \csname LTb\endcsname%
      \put(3411,2395){\makebox(0,0)[r]{\strut{}Trailing}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4972,552){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(4972,1224){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(4972,1896){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(4972,2568){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(4972,3240){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(5068,392){\makebox(0,0){\strut{}$0$}}%
      \put(6143,392){\makebox(0,0){\strut{}$10$}}%
      \put(7218,392){\makebox(0,0){\strut{}$20$}}%
      \put(8293,392){\makebox(0,0){\strut{}$30$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4508,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Vertical velocity $v/\sqrt{rg}$}}}%
      \put(6680,72){\makebox(0,0){\strut{}Time $t/\sqrt{r/g}$}}%
      \put(4472,4178){\makebox(0,0){\strut{}(b)}}%
      \csname LTb\endcsname%
      \put(7558,3595){\makebox(0,0)[r]{\strut{}Uhlmann leading}}%
      \csname LTb\endcsname%
      \put(7558,3355){\makebox(0,0)[r]{\strut{}Uhlmann trailing}}%
      \csname LTb\endcsname%
      \put(7558,3115){\makebox(0,0)[r]{\strut{}Glowinski leading}}%
      \csname LTb\endcsname%
      \put(7558,2875){\makebox(0,0)[r]{\strut{}Glowinski trailing}}%
      \csname LTb\endcsname%
      \put(7558,2635){\makebox(0,0)[r]{\strut{}Leading}}%
      \csname LTb\endcsname%
      \put(7558,2395){\makebox(0,0)[r]{\strut{}Trailing}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{dkt-traj_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> dkt-trajx.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9123.84,5529.60)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(641,671){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(641,1866){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(641,3061){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(737,392){\makebox(0,0){\strut{}$0$}}%
      \put(1812,392){\makebox(0,0){\strut{}$10$}}%
      \put(2887,392){\makebox(0,0){\strut{}$20$}}%
      \put(3962,392){\makebox(0,0){\strut{}$30$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(177,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Horizontal position $|x_c/r|$}}}%
      \put(2349,72){\makebox(0,0){\strut{}Time $t/\sqrt{r/g}$}}%
      \put(141,4178){\makebox(0,0){\strut{}(a)}}%
      \csname LTb\endcsname%
      \put(2678,3561){\makebox(0,0)[r]{\strut{}Uhlmann leading}}%
      \csname LTb\endcsname%
      \put(2678,3321){\makebox(0,0)[r]{\strut{}Uhlmann trailing}}%
      \csname LTb\endcsname%
      \put(2678,3081){\makebox(0,0)[r]{\strut{}Glowinski leading}}%
      \csname LTb\endcsname%
      \put(2678,2841){\makebox(0,0)[r]{\strut{}Glowinski trailing}}%
      \csname LTb\endcsname%
      \put(2678,2601){\makebox(0,0)[r]{\strut{}Leading}}%
      \csname LTb\endcsname%
      \put(2678,2361){\makebox(0,0)[r]{\strut{}Trailing}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4788,1013){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(4788,1935){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(4788,2856){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(4788,3778){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(4884,392){\makebox(0,0){\strut{}$0$}}%
      \put(5959,392){\makebox(0,0){\strut{}$10$}}%
      \put(7034,392){\makebox(0,0){\strut{}$20$}}%
      \put(8109,392){\makebox(0,0){\strut{}$30$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4420,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Horizontal velocity $|u/\sqrt{rg}|$}}}%
      \put(6496,72){\makebox(0,0){\strut{}Time $t/\sqrt{r/g}$}}%
      \put(4288,4178){\makebox(0,0){\strut{}(b)}}%
      \csname LTb\endcsname%
      \put(6825,3561){\makebox(0,0)[r]{\strut{}Uhlmann leading}}%
      \csname LTb\endcsname%
      \put(6825,3321){\makebox(0,0)[r]{\strut{}Uhlmann trailing}}%
      \csname LTb\endcsname%
      \put(6825,3081){\makebox(0,0)[r]{\strut{}Glowinski leading}}%
      \csname LTb\endcsname%
      \put(6825,2841){\makebox(0,0)[r]{\strut{}Glowinski trailing}}%
      \csname LTb\endcsname%
      \put(6825,2601){\makebox(0,0)[r]{\strut{}Leading}}%
      \csname LTb\endcsname%
      \put(6825,2361){\makebox(0,0)[r]{\strut{}Trailing}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{dkt-trajx_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> dkt.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9123.84,5990.40)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(456,1659){\makebox(0,0)[r]{\strut{}$-6$}}%
      \put(456,2949){\makebox(0,0)[r]{\strut{}$-4$}}%
      \put(456,4238){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(456,5528){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(746,1498){\makebox(0,0){\strut{}$-0.7$}}%
      \put(1649,1498){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(88,3593){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \put(1197,1258){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(591,5142){\makebox(0,0)[l]{\strut{}t=0s}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1857,1659){\makebox(0,0)[r]{\strut{}}}%
      \put(1857,2949){\makebox(0,0)[r]{\strut{}}}%
      \put(1857,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(1857,5528){\makebox(0,0)[r]{\strut{}}}%
      \put(2147,1498){\makebox(0,0){\strut{}$-0.7$}}%
      \put(3049,1498){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2598,1258){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(1992,5142){\makebox(0,0)[l]{\strut{}t=0.06s}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3258,1659){\makebox(0,0)[r]{\strut{}}}%
      \put(3258,2949){\makebox(0,0)[r]{\strut{}}}%
      \put(3258,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(3258,5528){\makebox(0,0)[r]{\strut{}}}%
      \put(3548,1498){\makebox(0,0){\strut{}$-0.7$}}%
      \put(4450,1498){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3999,1258){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(3393,5142){\makebox(0,0)[l]{\strut{}t=0.12s}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4659,1659){\makebox(0,0)[r]{\strut{}}}%
      \put(4659,2949){\makebox(0,0)[r]{\strut{}}}%
      \put(4659,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(4659,5528){\makebox(0,0)[r]{\strut{}}}%
      \put(4949,1498){\makebox(0,0){\strut{}$-0.7$}}%
      \put(5851,1498){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5400,1258){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(4794,5142){\makebox(0,0)[l]{\strut{}t=0.18s}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6060,1659){\makebox(0,0)[r]{\strut{}}}%
      \put(6060,2949){\makebox(0,0)[r]{\strut{}}}%
      \put(6060,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(6060,5528){\makebox(0,0)[r]{\strut{}}}%
      \put(6350,1498){\makebox(0,0){\strut{}$-0.7$}}%
      \put(7251,1498){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6800,1258){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(6195,5142){\makebox(0,0)[l]{\strut{}t=0.24s}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(7461,1659){\makebox(0,0)[r]{\strut{}}}%
      \put(7461,2949){\makebox(0,0)[r]{\strut{}}}%
      \put(7461,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(7461,5528){\makebox(0,0)[r]{\strut{}}}%
      \put(7751,1498){\makebox(0,0){\strut{}$-0.7$}}%
      \put(8652,1498){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(8201,1258){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(7596,5142){\makebox(0,0)[l]{\strut{}t=0.3s}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2396,385){\makebox(0,0){\strut{}$-200$}}%
      \put(3548,385){\makebox(0,0){\strut{}$-100$}}%
      \put(4700,385){\makebox(0,0){\strut{}$0$}}%
      \put(5851,385){\makebox(0,0){\strut{}$100$}}%
      \put(7003,385){\makebox(0,0){\strut{}$200$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1475,682){\makebox(0,0)[l]{\strut{}$\omega$ (s$^{-1}$)}}%
    }%
    \gplbacktext
    \put(552,1658){\includegraphics[width=64.55bp,height=193.55bp]{dkt_w_0}}%
    \put(1953,1658){\includegraphics[width=64.5bp,height=193.55bp]{dkt_w_100}}%
    \put(3354,1658){\includegraphics[width=64.5bp,height=193.55bp]{dkt_w_200}}%
    \put(4755,1658){\includegraphics[width=64.5bp,height=193.55bp]{dkt_w_300}}%
    \put(6156,1658){\includegraphics[width=64.45bp,height=193.55bp]{dkt_w_400}}%
    \put(7557,1658){\includegraphics[width=64.45bp,height=193.55bp]{dkt_w_500}}%
    \put(2396,552){\includegraphics[width=230.35bp,height=9.25bp]{dkt_wbar}}%
    \put(0,0){\includegraphics{dkt_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> five-star.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7257.60,8981.28)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(448,6260){\makebox(0,0)[r]{\strut{}$-1.4$}}%
      \put(448,6894){\makebox(0,0)[r]{\strut{}$-0.7$}}%
      \put(448,7529){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(448,8164){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(448,8798){\makebox(0,0)[r]{\strut{}$1.4$}}%
      \put(636,6008){\makebox(0,0){\strut{}}}%
      \put(1270,6008){\makebox(0,0){\strut{}}}%
      \put(1905,6008){\makebox(0,0){\strut{}}}%
      \put(2539,6008){\makebox(0,0){\strut{}}}%
      \put(3173,6008){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-116,7529){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \csname LTb\endcsname%
      \put(680,8618){\makebox(0,0)[l]{\strut{}$t=\SI{0}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3442,6260){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,6894){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,7529){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,8164){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,8798){\makebox(0,0)[r]{\strut{}}}%
      \put(3630,6008){\makebox(0,0){\strut{}}}%
      \put(4264,6008){\makebox(0,0){\strut{}}}%
      \put(4898,6008){\makebox(0,0){\strut{}}}%
      \put(5532,6008){\makebox(0,0){\strut{}}}%
      \put(6166,6008){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3674,8618){\makebox(0,0)[l]{\strut{}$t=\pi/25$~\si{s}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(448,3448){\makebox(0,0)[r]{\strut{}$-1.4$}}%
      \put(448,4082){\makebox(0,0)[r]{\strut{}$-0.7$}}%
      \put(448,4717){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(448,5352){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(448,5986){\makebox(0,0)[r]{\strut{}$1.4$}}%
      \put(636,3196){\makebox(0,0){\strut{}}}%
      \put(1270,3196){\makebox(0,0){\strut{}}}%
      \put(1905,3196){\makebox(0,0){\strut{}}}%
      \put(2539,3196){\makebox(0,0){\strut{}}}%
      \put(3173,3196){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-116,4717){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \csname LTb\endcsname%
      \put(680,5806){\makebox(0,0)[l]{\strut{}$t=2\pi/25$~\si{s}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3442,3448){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,4082){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,4717){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,5352){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,5986){\makebox(0,0)[r]{\strut{}}}%
      \put(3630,3196){\makebox(0,0){\strut{}}}%
      \put(4264,3196){\makebox(0,0){\strut{}}}%
      \put(4898,3196){\makebox(0,0){\strut{}}}%
      \put(5532,3196){\makebox(0,0){\strut{}}}%
      \put(6166,3196){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3674,5806){\makebox(0,0)[l]{\strut{}$t=3\pi/25$~\si{s}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(448,636){\makebox(0,0)[r]{\strut{}$-1.4$}}%
      \put(448,1270){\makebox(0,0)[r]{\strut{}$-0.7$}}%
      \put(448,1905){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(448,2540){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(448,3174){\makebox(0,0)[r]{\strut{}$1.4$}}%
      \put(636,384){\makebox(0,0){\strut{}$-1.4$}}%
      \put(1270,384){\makebox(0,0){\strut{}$-0.7$}}%
      \put(1905,384){\makebox(0,0){\strut{}$0$}}%
      \put(2539,384){\makebox(0,0){\strut{}$0.7$}}%
      \put(3173,384){\makebox(0,0){\strut{}$1.4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-116,1905){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \put(1904,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(680,2994){\makebox(0,0)[l]{\strut{}$t=4\pi/25$~\si{s}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3442,636){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,1270){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,1905){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,2540){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,3174){\makebox(0,0)[r]{\strut{}}}%
      \put(3630,384){\makebox(0,0){\strut{}$-1.4$}}%
      \put(4264,384){\makebox(0,0){\strut{}$-0.7$}}%
      \put(4898,384){\makebox(0,0){\strut{}$0$}}%
      \put(5532,384){\makebox(0,0){\strut{}$0.7$}}%
      \put(6166,384){\makebox(0,0){\strut{}$1.4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4898,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(3674,2994){\makebox(0,0)[l]{\strut{}$t=\pi/5$~\si{s}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6934,4626){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(6934,5987){\makebox(0,0)[l]{\strut{}$0.1$}}%
      \put(6934,7348){\makebox(0,0)[l]{\strut{}$0.2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6604,4354){\makebox(0,0)[l]{\strut{}$\|\mathbf{E}\|_F$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6934,997){\makebox(0,0)[l]{\strut{}$-100$}}%
      \put(6934,2358){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(6934,3719){\makebox(0,0)[l]{\strut{}$100$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6658,725){\makebox(0,0)[l]{\strut{}$\omega$ (s$^{-1}$)}}%
    }%
    \gplbacktext
    \put(544,6168){\includegraphics[width=136.05bp,height=136.1bp]{five-star_w_0}}%
    \put(3538,6168){\includegraphics[width=136bp,height=136.1bp]{five-star_w_80}}%
    \put(544,3356){\includegraphics[width=136.05bp,height=136.1bp]{five-star_w_160}}%
    \put(3538,3356){\includegraphics[width=136bp,height=136.1bp]{five-star_w_240}}%
    \put(544,544){\includegraphics[width=136.05bp,height=136.1bp]{five-star_w_320}}%
    \put(3538,544){\includegraphics[width=136bp,height=136.1bp]{five-star_w_400}}%
    \put(6622,4626){\includegraphics[width=9.05bp,height=136.1bp]{five-star_sbar}}%
    \put(6622,997){\includegraphics[width=9.05bp,height=136.1bp]{five-star_wbar}}%
    \put(0,0){\includegraphics{five-star_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> multi-drop.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8981.28,6350.40)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(448,3557){\makebox(0,0)[r]{\strut{}$-0.7$}}%
      \put(448,4445){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(448,5333){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(926,3015){\makebox(0,0){\strut{}}}%
      \put(1814,3015){\makebox(0,0){\strut{}}}%
      \put(2702,3015){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-116,4445){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \csname LTb\endcsname%
      \put(1179,5486){\makebox(0,0)[l]{\strut{}$t=\SI{0}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3079,3557){\makebox(0,0)[r]{\strut{}}}%
      \put(3079,4445){\makebox(0,0)[r]{\strut{}}}%
      \put(3079,5333){\makebox(0,0)[r]{\strut{}}}%
      \put(3557,3015){\makebox(0,0){\strut{}}}%
      \put(4445,3015){\makebox(0,0){\strut{}}}%
      \put(5332,3015){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3810,5486){\makebox(0,0)[l]{\strut{}$t=\SI{0.07}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5710,3557){\makebox(0,0)[r]{\strut{}}}%
      \put(5710,4445){\makebox(0,0)[r]{\strut{}}}%
      \put(5710,5333){\makebox(0,0)[r]{\strut{}}}%
      \put(6188,3015){\makebox(0,0){\strut{}}}%
      \put(7076,3015){\makebox(0,0){\strut{}}}%
      \put(7963,3015){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6441,5486){\makebox(0,0)[l]{\strut{}$t=\SI{0.14}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(448,926){\makebox(0,0)[r]{\strut{}$-0.7$}}%
      \put(448,1814){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(448,2702){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(926,384){\makebox(0,0){\strut{}$-0.7$}}%
      \put(1814,384){\makebox(0,0){\strut{}$0$}}%
      \put(2702,384){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-116,1814){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \put(1814,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(1179,2855){\makebox(0,0)[l]{\strut{}$t=\SI{0.21}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3079,926){\makebox(0,0)[r]{\strut{}}}%
      \put(3079,1814){\makebox(0,0)[r]{\strut{}}}%
      \put(3079,2702){\makebox(0,0)[r]{\strut{}}}%
      \put(3557,384){\makebox(0,0){\strut{}$-0.7$}}%
      \put(4445,384){\makebox(0,0){\strut{}$0$}}%
      \put(5332,384){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4444,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(3810,2855){\makebox(0,0)[l]{\strut{}$t=\SI{0.28}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5710,926){\makebox(0,0)[r]{\strut{}}}%
      \put(5710,1814){\makebox(0,0)[r]{\strut{}}}%
      \put(5710,2702){\makebox(0,0)[r]{\strut{}}}%
      \put(6188,384){\makebox(0,0){\strut{}$-0.7$}}%
      \put(7076,384){\makebox(0,0){\strut{}$0$}}%
      \put(7963,384){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7075,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(6441,2855){\makebox(0,0)[l]{\strut{}$t=\SI{0.35}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(8748,3719){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(8748,4324){\makebox(0,0)[l]{\strut{}$0.1$}}%
      \put(8748,4928){\makebox(0,0)[l]{\strut{}$0.2$}}%
      \put(8748,5533){\makebox(0,0)[l]{\strut{}$0.3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(8523,3356){\makebox(0,0)[l]{\strut{}$\|\mathbf{E}\|_F$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(8748,997){\makebox(0,0)[l]{\strut{}$-100$}}%
      \put(8748,1905){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(8748,2812){\makebox(0,0)[l]{\strut{}$100$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(8545,634){\makebox(0,0)[l]{\strut{}$\omega$ (s$^{-1}$)}}%
    }%
    \gplbacktext
    \put(544,3175){\includegraphics[width=127bp,height=127bp]{multi-drop_w_0}}%
    \put(3175,3175){\includegraphics[width=126.95bp,height=127bp]{multi-drop_w_100}}%
    \put(5806,3175){\includegraphics[width=126.95bp,height=127bp]{multi-drop_w_200}}%
    \put(544,544){\includegraphics[width=127bp,height=127bp]{multi-drop_w_300}}%
    \put(3175,544){\includegraphics[width=126.95bp,height=127bp]{multi-drop_w_400}}%
    \put(5806,544){\includegraphics[width=126.95bp,height=127bp]{multi-drop_w_500}}%
    \put(8527,3719){\includegraphics[width=4.5bp,height=90.7bp]{multi-drop_sbar}}%
    \put(8527,997){\includegraphics[width=4.5bp,height=90.75bp]{multi-drop_wbar}}%
    \put(0,0){\includegraphics{multi-drop_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> pentagon.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8981.28,6350.40)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(811,3178){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(811,4264){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(811,5349){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(910,3015){\makebox(0,0){\strut{}}}%
      \put(1996,3015){\makebox(0,0){\strut{}}}%
      \put(3081,3015){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(246,4263){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \csname LTb\endcsname%
      \put(972,5134){\makebox(0,0)[l]{\strut{}$t=\SI{0}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3396,3178){\makebox(0,0)[r]{\strut{}}}%
      \put(3396,4264){\makebox(0,0)[r]{\strut{}}}%
      \put(3396,5349){\makebox(0,0)[r]{\strut{}}}%
      \put(3495,3015){\makebox(0,0){\strut{}}}%
      \put(4581,3015){\makebox(0,0){\strut{}}}%
      \put(5666,3015){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3557,5134){\makebox(0,0)[l]{\strut{}$t=\SI{0.04}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5982,3178){\makebox(0,0)[r]{\strut{}}}%
      \put(5982,4264){\makebox(0,0)[r]{\strut{}}}%
      \put(5982,5349){\makebox(0,0)[r]{\strut{}}}%
      \put(6081,3015){\makebox(0,0){\strut{}}}%
      \put(7166,3015){\makebox(0,0){\strut{}}}%
      \put(8251,3015){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6143,5134){\makebox(0,0)[l]{\strut{}$t=\SI{0.08}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(811,547){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(811,1633){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(811,2718){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(910,384){\makebox(0,0){\strut{}$-0.5$}}%
      \put(1996,384){\makebox(0,0){\strut{}$0$}}%
      \put(3081,384){\makebox(0,0){\strut{}$0.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(246,1632){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \put(1995,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(972,2503){\makebox(0,0)[l]{\strut{}$t=\SI{0.12}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3396,547){\makebox(0,0)[r]{\strut{}}}%
      \put(3396,1633){\makebox(0,0)[r]{\strut{}}}%
      \put(3396,2718){\makebox(0,0)[r]{\strut{}}}%
      \put(3495,384){\makebox(0,0){\strut{}$-0.5$}}%
      \put(4581,384){\makebox(0,0){\strut{}$0$}}%
      \put(5666,384){\makebox(0,0){\strut{}$0.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4580,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(4707,2503){\makebox(0,0)[l]{\strut{}$t=\SI{0.16}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5982,547){\makebox(0,0)[r]{\strut{}}}%
      \put(5982,1633){\makebox(0,0)[r]{\strut{}}}%
      \put(5982,2718){\makebox(0,0)[r]{\strut{}}}%
      \put(6081,384){\makebox(0,0){\strut{}$-0.5$}}%
      \put(7166,384){\makebox(0,0){\strut{}$0$}}%
      \put(8251,384){\makebox(0,0){\strut{}$0.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7166,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(6143,2503){\makebox(0,0)[l]{\strut{}$t=\SI{0.2}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(8703,1451){\makebox(0,0)[l]{\strut{}$-60$}}%
      \put(8703,3266){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(8703,5080){\makebox(0,0)[l]{\strut{}$60$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(8500,1088){\makebox(0,0)[l]{\strut{}$\omega (s^{-1})$}}%
    }%
    \gplbacktext
    \put(907,3175){\includegraphics[width=108.85bp,height=108.85bp]{pentagon_w_0}}%
    \put(3492,3175){\includegraphics[width=108.85bp,height=108.85bp]{pentagon_w_80}}%
    \put(6078,3175){\includegraphics[width=108.8bp,height=108.85bp]{pentagon_w_160}}%
    \put(907,544){\includegraphics[width=108.85bp,height=108.85bp]{pentagon_w_240}}%
    \put(3492,544){\includegraphics[width=108.85bp,height=108.85bp]{pentagon_w_320}}%
    \put(6078,544){\includegraphics[width=108.8bp,height=108.85bp]{pentagon_w_400}}%
    \put(8482,1451){\includegraphics[width=4.5bp,height=181.45bp]{pentagon_wbar}}%
    \put(0,0){\includegraphics{pentagon_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> rod-drop.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8981.28,8981.28)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(811,4628){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(811,5897){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(811,7165){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(811,8434){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1162,4466){\makebox(0,0){\strut{}}}%
      \put(1669,4466){\makebox(0,0){\strut{}}}%
      \put(2177,4466){\makebox(0,0){\strut{}}}%
      \put(2684,4466){\makebox(0,0){\strut{}}}%
      \put(3191,4466){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(438,6531){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \csname LTb\endcsname%
      \put(983,8246){\makebox(0,0)[l]{\strut{}$t=\SI{0}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3442,4628){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,5897){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,7165){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,8434){\makebox(0,0)[r]{\strut{}}}%
      \put(3793,4466){\makebox(0,0){\strut{}}}%
      \put(4300,4466){\makebox(0,0){\strut{}}}%
      \put(4808,4466){\makebox(0,0){\strut{}}}%
      \put(5315,4466){\makebox(0,0){\strut{}}}%
      \put(5822,4466){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3614,8246){\makebox(0,0)[l]{\strut{}$t=\SI{0.125}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6072,4628){\makebox(0,0)[r]{\strut{}}}%
      \put(6072,5897){\makebox(0,0)[r]{\strut{}}}%
      \put(6072,7165){\makebox(0,0)[r]{\strut{}}}%
      \put(6072,8434){\makebox(0,0)[r]{\strut{}}}%
      \put(6423,4466){\makebox(0,0){\strut{}}}%
      \put(6931,4466){\makebox(0,0){\strut{}}}%
      \put(7438,4466){\makebox(0,0){\strut{}}}%
      \put(7945,4466){\makebox(0,0){\strut{}}}%
      \put(8453,4466){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6244,8246){\makebox(0,0)[l]{\strut{}$t=\SI{0.25}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(811,546){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(811,1815){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(811,3083){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(811,4352){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1162,384){\makebox(0,0){\strut{}$-0.8$}}%
      \put(1669,384){\makebox(0,0){\strut{}$-0.4$}}%
      \put(2177,384){\makebox(0,0){\strut{}$0$}}%
      \put(2684,384){\makebox(0,0){\strut{}$0.4$}}%
      \put(3191,384){\makebox(0,0){\strut{}$0.8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(438,2449){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \put(2176,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(983,4164){\makebox(0,0)[l]{\strut{}$t=\SI{0.375}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3442,546){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,1815){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,3083){\makebox(0,0)[r]{\strut{}}}%
      \put(3442,4352){\makebox(0,0)[r]{\strut{}}}%
      \put(3793,384){\makebox(0,0){\strut{}$-0.8$}}%
      \put(4300,384){\makebox(0,0){\strut{}$-0.4$}}%
      \put(4808,384){\makebox(0,0){\strut{}$0$}}%
      \put(5315,384){\makebox(0,0){\strut{}$0.4$}}%
      \put(5822,384){\makebox(0,0){\strut{}$0.8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4807,144){\makebox(0,0){\strut{}$x$ (cm)}}%
      \csname LTb\endcsname%
      \put(3614,4164){\makebox(0,0)[l]{\strut{}$t=\SI{0.5}{s}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6934,997){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(6934,2585){\makebox(0,0)[l]{\strut{}$1$}}%
      \put(6934,4173){\makebox(0,0)[l]{\strut{}$2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6522,679){\makebox(0,0)[l]{\strut{}$\|\mathbf{E}\|_F$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(8294,997){\makebox(0,0)[l]{\strut{}$-200$}}%
      \put(8294,1791){\makebox(0,0)[l]{\strut{}$-100$}}%
      \put(8294,2585){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(8294,3379){\makebox(0,0)[l]{\strut{}$100$}}%
      \put(8294,4173){\makebox(0,0)[l]{\strut{}$200$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7893,679){\makebox(0,0)[l]{\strut{}$\omega$ (s$^{-1}$)}}%
    }%
    \gplbacktext
    \put(907,4626){\includegraphics[width=126.95bp,height=190.5bp]{rod-drop_w_0}}%
    \put(3538,4626){\includegraphics[width=126.95bp,height=190.5bp]{rod-drop_w_50}}%
    \put(6168,4626){\includegraphics[width=127bp,height=190.5bp]{rod-drop_w_100}}%
    \put(907,544){\includegraphics[width=126.95bp,height=190.5bp]{rod-drop_w_150}}%
    \put(3538,544){\includegraphics[width=126.95bp,height=190.5bp]{rod-drop_w_200}}%
    \put(6622,997){\includegraphics[width=9.05bp,height=158.8bp]{rod-drop_sbar}}%
    \put(7983,997){\includegraphics[width=9bp,height=158.8bp]{rod-drop_wbar}}%
    \put(0,0){\includegraphics{rod-drop_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> single-drop.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9123.84,5529.60)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(456,1475){\makebox(0,0)[r]{\strut{}$-8$}}%
      \put(456,2396){\makebox(0,0)[r]{\strut{}$-6$}}%
      \put(456,3317){\makebox(0,0)[r]{\strut{}$-4$}}%
      \put(456,4238){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(456,5159){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(691,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(1335,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(21,3317){\rotatebox{-270}{\makebox(0,0){\strut{}$y$ (cm)}}}%
      \put(1013,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \put(725,5400){\makebox(0,0){\strut{}(a)}}%
      \csname LTb\endcsname%
      \put(598,4791){\makebox(0,0)[l]{\strut{}\scriptsize $G=10$ Pa}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1470,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(1470,2396){\makebox(0,0)[r]{\strut{}}}%
      \put(1470,3317){\makebox(0,0)[r]{\strut{}}}%
      \put(1470,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(1470,5159){\makebox(0,0)[r]{\strut{}}}%
      \put(1705,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(2349,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2027,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \put(1739,5080){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1612,4791){\makebox(0,0)[l]{\strut{}\scriptsize $G=100$ Pa}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2484,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(2484,2396){\makebox(0,0)[r]{\strut{}}}%
      \put(2484,3317){\makebox(0,0)[r]{\strut{}}}%
      \put(2484,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(2484,5159){\makebox(0,0)[r]{\strut{}}}%
      \put(2719,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(3362,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3040,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \put(2752,5080){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(2626,4791){\makebox(0,0)[l]{\strut{}\scriptsize \shortstack[l]{$G=$\\ $1000$ Pa}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3498,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(3498,2396){\makebox(0,0)[r]{\strut{}}}%
      \put(3498,3317){\makebox(0,0)[r]{\strut{}}}%
      \put(3498,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(3498,5159){\makebox(0,0)[r]{\strut{}}}%
      \put(3733,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(4376,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4054,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \put(3766,5080){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(3640,4791){\makebox(0,0)[l]{\strut{}\scriptsize Rigid}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4696,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(4696,2396){\makebox(0,0)[r]{\strut{}}}%
      \put(4696,3317){\makebox(0,0)[r]{\strut{}}}%
      \put(4696,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(4696,5159){\makebox(0,0)[r]{\strut{}}}%
      \put(4931,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(5574,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5252,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \put(4964,5400){\makebox(0,0){\strut{}(b)}}%
      \csname LTb\endcsname%
      \put(4838,4791){\makebox(0,0)[l]{\strut{}\scriptsize $G=10$ Pa}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5710,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(5710,2396){\makebox(0,0)[r]{\strut{}}}%
      \put(5710,3317){\makebox(0,0)[r]{\strut{}}}%
      \put(5710,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(5710,5159){\makebox(0,0)[r]{\strut{}}}%
      \put(5944,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(6588,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6266,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \put(5978,5080){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(5852,4791){\makebox(0,0)[l]{\strut{}\scriptsize $G=100$ Pa}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6723,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(6723,2396){\makebox(0,0)[r]{\strut{}}}%
      \put(6723,3317){\makebox(0,0)[r]{\strut{}}}%
      \put(6723,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(6723,5159){\makebox(0,0)[r]{\strut{}}}%
      \put(6958,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(7601,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7279,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \put(6991,5080){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(6865,4791){\makebox(0,0)[l]{\strut{}\scriptsize \shortstack[l]{ $G=$\\$1000$ Pa}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(7737,1475){\makebox(0,0)[r]{\strut{}}}%
      \put(7737,2396){\makebox(0,0)[r]{\strut{}}}%
      \put(7737,3317){\makebox(0,0)[r]{\strut{}}}%
      \put(7737,4238){\makebox(0,0)[r]{\strut{}}}%
      \put(7737,5159){\makebox(0,0)[r]{\strut{}}}%
      \put(7972,1314){\makebox(0,0){\strut{}$-0.7$}}%
      \put(8615,1314){\makebox(0,0){\strut{}$0.7$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(8293,1074){\makebox(0,0){\strut{}$x$ (cm)}}%
      \put(8005,5080){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(7879,4791){\makebox(0,0)[l]{\strut{}\scriptsize Rigid}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2396,385){\makebox(0,0){\strut{}$-100$}}%
      \put(4700,385){\makebox(0,0){\strut{}$0$}}%
      \put(7003,385){\makebox(0,0){\strut{}$100$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4411,817){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%
      \put(1475,663){\makebox(0,0)[l]{\strut{}$\omega$ (s$^{-1})$}}%
    }%
    \gplbacktext
    \put(552,1474){\includegraphics[width=46.1bp,height=184.3bp]{circle-drop_w_1}}%
    \put(1566,1474){\includegraphics[width=46.1bp,height=184.3bp]{circle-drop_w_10}}%
    \put(2580,1474){\includegraphics[width=46.05bp,height=184.3bp]{circle-drop_w_100}}%
    \put(3594,1474){\includegraphics[width=46.05bp,height=184.3bp]{circle-drop_w_1000}}%
    \put(4792,1474){\includegraphics[width=46.05bp,height=184.3bp]{square-drop_w_1}}%
    \put(5806,1474){\includegraphics[width=46bp,height=184.3bp]{square-drop_w_10}}%
    \put(6819,1474){\includegraphics[width=46.05bp,height=184.3bp]{square-drop_w_100}}%
    \put(7833,1474){\includegraphics[width=46.05bp,height=184.3bp]{square-drop_w_1000}}%
    \put(2396,552){\includegraphics[width=230.35bp,height=9.25bp]{square-drop_wbar}}%
    \put(0,0){\includegraphics{single-drop_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> singleobj.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9123.84,9123.84)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(825,5160){\makebox(0,0)[r]{\strut{}$-8$}}%
      \put(825,5967){\makebox(0,0)[r]{\strut{}$-6$}}%
      \put(825,6773){\makebox(0,0)[r]{\strut{}$-4$}}%
      \put(825,7580){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(825,8386){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(921,5000){\makebox(0,0){\strut{}$0$}}%
      \put(1842,5000){\makebox(0,0){\strut{}$0.1$}}%
      \put(2764,5000){\makebox(0,0){\strut{}$0.2$}}%
      \put(3685,5000){\makebox(0,0){\strut{}$0.3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(361,6773){\rotatebox{-270}{\makebox(0,0){\strut{}Vertical center of mass location $y_c$ (cm)}}}%
      \put(2533,4760){\makebox(0,0){\strut{}Time $t$ (s)}}%
      \put(613,8946){\makebox(0,0){\strut{}(a)}}%
      \csname LTb\endcsname%
      \put(3699,8205){\makebox(0,0)[r]{\strut{}$G=10$ Pa}}%
      \csname LTb\endcsname%
      \put(3699,7969){\makebox(0,0)[r]{\strut{}$G=100$ Pa}}%
      \csname LTb\endcsname%
      \put(3699,7733){\makebox(0,0)[r]{\strut{}$G=1000$ Pa}}%
      \csname LTb\endcsname%
      \put(3699,7497){\makebox(0,0)[r]{\strut{}Rigid}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5433,5160){\makebox(0,0)[r]{\strut{}$-20$}}%
      \put(5433,6235){\makebox(0,0)[r]{\strut{}$-10$}}%
      \put(5433,7311){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(5433,8386){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(5529,5000){\makebox(0,0){\strut{}$0$}}%
      \put(6450,5000){\makebox(0,0){\strut{}$0.1$}}%
      \put(7372,5000){\makebox(0,0){\strut{}$0.2$}}%
      \put(8293,5000){\makebox(0,0){\strut{}$0.3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4800,6773){\rotatebox{-270}{\makebox(0,0){\strut{}Vertical velocity $v$ (cm/s)}}}%
      \put(7141,4760){\makebox(0,0){\strut{}Time $t$ (s)}}%
      \put(5221,8946){\makebox(0,0){\strut{}(b)}}%
      \csname LTb\endcsname%
      \put(8307,8205){\makebox(0,0)[r]{\strut{}$G=10$ Pa}}%
      \csname LTb\endcsname%
      \put(8307,7969){\makebox(0,0)[r]{\strut{}$G=100$ Pa}}%
      \csname LTb\endcsname%
      \put(8307,7733){\makebox(0,0)[r]{\strut{}$G=1000$ Pa}}%
      \csname LTb\endcsname%
      \put(8307,7497){\makebox(0,0)[r]{\strut{}Rigid}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(825,552){\makebox(0,0)[r]{\strut{}$-8$}}%
      \put(825,1359){\makebox(0,0)[r]{\strut{}$-6$}}%
      \put(825,2165){\makebox(0,0)[r]{\strut{}$-4$}}%
      \put(825,2972){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(825,3778){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(921,392){\makebox(0,0){\strut{}$0$}}%
      \put(1842,392){\makebox(0,0){\strut{}$0.1$}}%
      \put(2764,392){\makebox(0,0){\strut{}$0.2$}}%
      \put(3685,392){\makebox(0,0){\strut{}$0.3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(361,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Vertical center of mass location $y_c$ (cm)}}}%
      \put(2533,152){\makebox(0,0){\strut{}Time $t$ (s)}}%
      \put(613,4338){\makebox(0,0){\strut{}(c)}}%
      \csname LTb\endcsname%
      \put(3699,3597){\makebox(0,0)[r]{\strut{}$G=10$ Pa}}%
      \csname LTb\endcsname%
      \put(3699,3361){\makebox(0,0)[r]{\strut{}$G=100$ Pa}}%
      \csname LTb\endcsname%
      \put(3699,3125){\makebox(0,0)[r]{\strut{}$G=1000$ Pa}}%
      \csname LTb\endcsname%
      \put(3699,2889){\makebox(0,0)[r]{\strut{}Rigid}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5433,552){\makebox(0,0)[r]{\strut{}$-20$}}%
      \put(5433,1627){\makebox(0,0)[r]{\strut{}$-10$}}%
      \put(5433,2703){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(5433,3778){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(5529,392){\makebox(0,0){\strut{}$0$}}%
      \put(6450,392){\makebox(0,0){\strut{}$0.1$}}%
      \put(7372,392){\makebox(0,0){\strut{}$0.2$}}%
      \put(8293,392){\makebox(0,0){\strut{}$0.3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4800,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Vertical velocity $v$ (cm/s)}}}%
      \put(7141,152){\makebox(0,0){\strut{}Time $t$ (s)}}%
      \put(5221,4338){\makebox(0,0){\strut{}(d)}}%
      \csname LTb\endcsname%
      \put(8307,3597){\makebox(0,0)[r]{\strut{}$G=10$ Pa}}%
      \csname LTb\endcsname%
      \put(8307,3361){\makebox(0,0)[r]{\strut{}$G=100$ Pa}}%
      \csname LTb\endcsname%
      \put(8307,3125){\makebox(0,0)[r]{\strut{}$G=1000$ Pa}}%
      \csname LTb\endcsname%
      \put(8307,2889){\makebox(0,0)[r]{\strut{}Rigid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{singleobj_a}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> visc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9123.84,5529.60)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(825,1013){\makebox(0,0)[r]{\strut{}$-0.3$}}%
      \put(825,1935){\makebox(0,0)[r]{\strut{}$-0.2$}}%
      \put(825,2856){\makebox(0,0)[r]{\strut{}$-0.1$}}%
      \put(825,3778){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(921,392){\makebox(0,0){\strut{}$0$}}%
      \put(1842,392){\makebox(0,0){\strut{}$2$}}%
      \put(2764,392){\makebox(0,0){\strut{}$4$}}%
      \put(3685,392){\makebox(0,0){\strut{}$6$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(169,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Vertical velocity $v/\sqrt{dg}$}}}%
      \put(2533,72){\makebox(0,0){\strut{}Time $t/\sqrt{d/g}$ }}%
      \put(613,4178){\makebox(0,0){\strut{}(a)}}%
      \csname LTb\endcsname%
      \put(3411,3595){\makebox(0,0)[r]{\strut{}$50\times 200$}}%
      \csname LTb\endcsname%
      \put(3411,3355){\makebox(0,0)[r]{\strut{}$100 \times 400$}}%
      \csname LTb\endcsname%
      \put(3411,3115){\makebox(0,0)[r]{\strut{}$200 \times 800$}}%
      \csname LTb\endcsname%
      \put(3411,2875){\makebox(0,0)[r]{\strut{}Analytical}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(5433,932){\makebox(0,0)[r]{\strut{}$-0.15$}}%
      \put(5433,1880){\makebox(0,0)[r]{\strut{}$-0.1$}}%
      \put(5433,2829){\makebox(0,0)[r]{\strut{}$-0.05$}}%
      \put(5433,3778){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(5529,392){\makebox(0,0){\strut{}$0$}}%
      \put(6174,392){\makebox(0,0){\strut{}$1$}}%
      \put(6819,392){\makebox(0,0){\strut{}$2$}}%
      \put(7464,392){\makebox(0,0){\strut{}$3$}}%
      \put(8109,392){\makebox(0,0){\strut{}$4$}}%
      \put(8754,392){\makebox(0,0){\strut{}$5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4681,2165){\rotatebox{-270}{\makebox(0,0){\strut{}Vertical velocity $v/\sqrt{dg}$}}}%
      \put(7141,72){\makebox(0,0){\strut{}Time $t/\sqrt{d/g}$}}%
      \put(5221,4178){\makebox(0,0){\strut{}(b)}}%
      \csname LTb\endcsname%
      \put(8019,3595){\makebox(0,0)[r]{\strut{}$50\times 200$}}%
      \csname LTb\endcsname%
      \put(8019,3355){\makebox(0,0)[r]{\strut{}$100 \times 400$}}%
      \csname LTb\endcsname%
      \put(8019,3115){\makebox(0,0)[r]{\strut{}$200 \times 800$}}%
      \csname LTb\endcsname%
      \put(8019,2875){\makebox(0,0)[r]{\strut{}Analytical}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{visc_a}}%
    \gplfronttext
  \end{picture}%
\endgroup

